SoK: DAG-based Consensus Protocols

This paper is a Systematization of Knowledge (SoK) on Directed Acyclic Graph (DAG)-based consensus protocols, analyzing their performance and trade-offs within the framework of consistency, availability, and partition tolerance inspired by the CAP theorem. We classify DAG-based consensus protocols into availability-focused and consistency-focused categories, exploring their design principles, core functionalities, and associated trade-offs. Furthermore, we examine key properties, attack vectors, and recent developments, providing insights into security, scalability, and fairness challenges. Finally, we identify research gaps and outline directions for advancing DAG-based consensus mechanisms.

==> DAGsrelation.tex <==
\begin{tikzpicture}[scale=0.1,
    block/.style={draw, fill=blue!20, rectangle, minimum height=3em, minimum width=6em, align=center},
    line/.style={draw, -{Triangle[width=9pt,length=4pt]}, shorten >=1pt},
    auto,
    node distance=1.5cm
]

    % Define styles for different types of lines
    \tikzset{
        dash line/.style={draw, dashed, -{Triangle[width=9pt,length=4pt]}, shorten >=1pt}
    }
    
   
 % Nodes for Certified DAG
    \node [block, fill=green!20] (certifiedDAG) {Certified DAG};
    \node [block, right=of certifiedDAG] (aleph) {Aleph\\(2018)};
    \node [block, right=of aleph] (dagRider) {DAG Rider\\(2021)};
    
    \node [block, right=of dagRider, xshift=-0.6cm] (narwhalTusk) {Narwhal and\\Tusk\\(2021)};
    \node [block, right=of narwhalTusk, xshift=-0.6cm] (bullshark) {Bullshark\\(2022)};
    \node [block, right=of bullshark] (shoal) {Shoal\\(2023)};
    
    \node [block, right=of shoal, xshift=0.5cm, yshift=1cm] (sailfish) {Sailfish\\(2024)}; 
    \node [block, right=of shoal, xshift=-0.2cm, yshift=-1.5cm] (bbca) {BBCA-Chain\\(2023)};


% Nodes for Fast payment
    \node [block, fill=yellow!20, below=of certifiedDAG] (fastPayment) {Fast payment};
    \node [block, right=of fastPayment, xshift=2cm] (fastpay) {Fastpay\\(2020)};
    \node [block, right=of fastpay, xshift=7.2cm] (flash) {Flash\\(2023)};
    \node[block, below=of bbca,  yshift=1cm] (mysticeti) {Mysticeti\\(2023)};
  

% Nodes for Optimistic DAG
    \node [block, fill=blue!40, below=of fastPayment] (optimisticDAG) {Optimistic DAG};
    \node [block, right=of optimisticDAG, xshift=-0.5cm, yshift=1cm] (hashgraph) {Hashgraph\\(2016)};
    \node [block, right=of hashgraph, xshift=6.8cm] (cordialMiners) {Cordial Miners\\(2022)};
    \node [block, below=of hashgraph, xshift=0.3cm] (iota) {IOTA\\(2017-now)};
    \node [block, right=of iota, , xshift=9.5cm] (iota2) {IOTA 2.0\\(2023)};


%% % % % %  %% % % % % %% % % % %  

  
  % Lines for Certified DAG
    \draw [line] (certifiedDAG) -- (aleph);
    \draw [dash line] (aleph) -- (dagRider);
    
    \draw [line] (dagRider) -- (narwhalTusk);
    \draw [line] (narwhalTusk) -- (bullshark);
    \draw [line] (bullshark) -- (shoal);
    \draw [line] (shoal) -- (sailfish);
    \draw [line] (shoal) -- (bbca);

      
%% % % % %  %% % % % % %% % % % %  


    % Lines for Fast payment
    \draw [line] (fastPayment) -- (fastpay);
    \draw [dash line] (fastpay) -- (flash);
    \draw [dash line] (flash) -- (bbca);
    \draw [dash line] (flash) -- (mysticeti);
    

%% % % % %  %% % % % % %% % % % % 

    % Lines for Optimistic DAG
    \draw [line] (optimisticDAG) -- (hashgraph);
    \draw [dash line] (hashgraph) -- (cordialMiners);
    \draw [line] (optimisticDAG) -- (iota);
    \draw [line] (iota) -- (iota2);
    \draw [dash line] (hashgraph) -- (iota2);
    \draw [line] (cordialMiners) -- (mysticeti);
    \draw [dash line] (iota2) -- (mysticeti);

 
% Background coloring for Certified DAG Section
    % \begin{scope}[on background layer]
    %     \fill[green!20] ($(certifiedDAG.north west)+(0,1.5)$) rectangle ($(sailfish.south east)+(0,-2.5)$);
    % \end{scope}


% % Background coloring for Fast payment Section
% \begin{scope}[on background layer]
%     \fill[blue!20] (fastPayment.north -| fastPayment.west) rectangle (flash.south -| flash.east);
% \end{scope} 
 
    % Lines
    % \draw [line] (certifiedDAG.east) -- (aleph.west);
    % \draw [line] (fastPayment.east) -- (fastpay.west);
    % \draw [line] (optimisticDAG.east) -- (hashgraph.west);
    % ... add more lines here


% % Background coloring for Optimistic DAG Section
% \begin{scope}[on background layer]
%     \fill[blue!40] (optimisticDAG.north -| optimisticDAG.west) rectangle (iota2.south -| iota2.east);
% \end{scope}    % ... more background coloring for other sections



    % Labels, such as title
% Add label at the top for "Evolution of DAG-based protocols"
%    \node [above=of certifiedDAG, font=\Large\bfseries] {Evolution of DAG-based protocols (with deterministic finality)};

\end{tikzpicture}

==> conesInUnstructuredDAG.tex <==
%\tikzstyle{block_marking_red}[draw=red, thick, rounded corners=.1cm, inner sep=1pt]
\begin{figure}[t]
    \centering
\begin{tikzpicture}
% Block scheme
\def\xCoordinate{0.0}
\def\yCoordinate{0.0}
\def\yAdd{1.5}
\def\xAdd{0.75}
\def\innerSepar{-1.5}
\def\lineWidth{1.5}
\def\roundedCorners{1}
\def\opacityInternal{0.5}
\def\minHeight{20}
\def\minWidth{20}
\tikzstyle{block}=[draw, rectangle, minimum height=\minHeight pt, minimum width = \minWidth pt, text centered, rounded corners=\roundedCorners pt, draw=darkgray, font=\large]
\def\arrowStyle{-latex}
\node[block] (central_block) at (\xCoordinate,\yCoordinate) {$x$};
 \node [draw=red,opacity=\opacityInternal,rounded corners= \roundedCorners pt,line width = \lineWidth pt,
        inner sep=\innerSepar pt,fit=(central_block)] (red_central_block) {};
 \node [draw=blue, opacity=\opacityInternal, rounded corners =  \roundedCorners pt,line width = \lineWidth pt,
        inner sep=\innerSepar pt,fit=(red_central_block)] (blue_central_block) {};
        
\node[block] (blue_below_1_1) at (\xCoordinate-\xAdd,\yCoordinate-\yAdd) {};
 \node [draw=blue,opacity=\opacityInternal,rounded corners= \roundedCorners pt,line width = \lineWidth pt,
        inner sep=\innerSepar pt,fit=(blue_below_1_1)] (blue_blue_below_1_1) {};
 \draw[\arrowStyle] (blue_below_1_1) -- (central_block);  

\node[block] (blue_below_1_2) at (\xCoordinate+\xAdd,\yCoordinate-\yAdd) {};
 \node [draw=blue,opacity=\opacityInternal,rounded corners= \roundedCorners pt,line width = \lineWidth pt,
        inner sep=\innerSepar pt,fit=(blue_below_1_2)] (blue_blue_below_1_2) {};
 \draw[\arrowStyle] (blue_below_1_2) -- (central_block); 
 
 
 %\node[block] (blue_below_2_0) at (\xCoordinate-2*\xAdd,\yCoordinate-2*\yAdd) {};
 %\node [draw=blue,opacity=\opacityInternal,rounded corners= \roundedCorners pt,line width = \lineWidth pt,
 %       inner sep=\innerSepar pt,fit=(blue_below_2_0)] (blue_blue_below_2_0) {};
 %\draw[\arrowStyle] (blue_below_2_0) -- (blue_below_1_1); 
 
 \node[block] (blue_below_2_1) at (\xCoordinate,\yCoordinate-2*\yAdd) {};
 \node [draw=blue,opacity=\opacityInternal,rounded corners= \roundedCorners pt,line width = \lineWidth pt,
        inner sep=\innerSepar pt,fit=(blue_below_2_1)] (blue_blue_below_2_1) {};
 \draw[\arrowStyle] (blue_below_2_1) -- (blue_below_1_2); 
 \draw[\arrowStyle] (blue_below_2_1) -- (blue_below_1_1); 
 
 \node[block] (blue_below_2_2) at (\xCoordinate+2*\xAdd,\yCoordinate-2*\yAdd) {};
 \node [draw=blue,opacity=\opacityInternal,rounded corners= \roundedCorners pt,line width = \lineWidth pt,
        inner sep=\innerSepar pt,fit=(blue_below_2_2)] (blue_blue_below_2_2) {};
 \draw[\arrowStyle] (blue_below_2_2) -- (blue_below_1_2); 
 \draw[\arrowStyle, path fading = south]  (\xCoordinate,\yCoordinate-3*\yAdd) -- (blue_below_2_2) ; 
 \draw[\arrowStyle, path fading = south]  (\xCoordinate-3*\xAdd,\yCoordinate-3*\yAdd) -- (blue_below_2_1) ; 
 
 \draw[\arrowStyle, path fading = south]  (\xCoordinate+3*\xAdd,\yCoordinate-3*\yAdd) -- (blue_below_2_2) ; 
 
 
 \node[block] (red_above_1) at (\xCoordinate,\yCoordinate+\yAdd) {};
 \node [draw=red,opacity=\opacityInternal,rounded corners= \roundedCorners pt,line width = \lineWidth pt,
        inner sep=\innerSepar pt,fit=(red_above_1)] (red_red_above_1) {};
 \draw[\arrowStyle] (central_block) -- (red_above_1);

  \node[block] (red_above_2_1) at (\xCoordinate+\xAdd,\yCoordinate+2*\yAdd) {};
  \draw[\arrowStyle] (red_above_1) -- (red_above_2_1);
   \node [draw=red,opacity=\opacityInternal,rounded corners= \roundedCorners pt,line width = \lineWidth pt,
        inner sep=\innerSepar pt,fit=(red_above_2_1)] (red_red_above_2_1) {};
  
  \node[block] (red_above_2_2) at (\xCoordinate-\xAdd,\yCoordinate+2*\yAdd) {};
  \node [draw=red,opacity=\opacityInternal,rounded corners= \roundedCorners pt,line width = \lineWidth pt,
        inner sep=\innerSepar pt,fit=(red_above_2_2)] (red_red_above_2_2) {};
  \draw[\arrowStyle] (red_above_1) -- (red_above_2_2);
  
  
  \node[block] (red_above_3) at (\xCoordinate,\yCoordinate+3*\yAdd) {};
   \node [draw=red,opacity=\opacityInternal,rounded corners= \roundedCorners pt,line width = \lineWidth pt,
        inner sep=\innerSepar pt,fit=(red_above_3)] (red_red_above_3) {};
  \draw[\arrowStyle] (red_above_2_2) -- (red_above_3);
  \draw[\arrowStyle] (red_above_2_1) -- (red_above_3);

 \node[block] (red_above_3_0) at (\xCoordinate-2*\xAdd,\yCoordinate+3*\yAdd) {};
   \node [draw=red,opacity=\opacityInternal,rounded corners= \roundedCorners pt,line width = \lineWidth pt,
        inner sep=\innerSepar pt,fit=(red_above_3_0)] (red_red_above_3_0) {};
  \draw[\arrowStyle] (red_above_2_2) -- (red_above_3_0);
  \draw[\arrowStyle] (red_above_2_1) -- (red_above_3);
 \draw[\arrowStyle,path fading=north] (red_above_3) -- (\xCoordinate,\yCoordinate+4*\yAdd);
  \draw[\arrowStyle,path fading=north] (red_above_3_0) -- (\xCoordinate-\xAdd,\yCoordinate+4*\yAdd);
  \draw[\arrowStyle,path fading=north] (red_above_3_0) -- (\xCoordinate-2*\xAdd,\yCoordinate+4*\yAdd);
  

\node[block] (central_grey_left) at (\xCoordinate-2*\xAdd,\yCoordinate) {};
 \draw[\arrowStyle] (central_grey_left) -- (red_above_1);  
 
\node[block] (central_grey_right) at (\xCoordinate+2*\xAdd,\yCoordinate) {}; 

 \draw[\arrowStyle] (central_grey_right) -- (red_above_2_1);
 \draw[\arrowStyle] (blue_below_1_2) -- (central_grey_right);

 
 \node[block] (above_grey_1) at (\xCoordinate-3*\xAdd,\yCoordinate+\yAdd) {};
 \draw[\arrowStyle] (above_grey_1) -- (red_above_2_2);
\draw[\arrowStyle] (central_grey_left) -- (above_grey_1);
\draw[\arrowStyle] (blue_below_1_1) -- (central_grey_left);
\draw[\arrowStyle] (above_grey_1) -- (red_above_3_0);


 \node[block] (below_grey_1) at (\xCoordinate-3*\xAdd,\yCoordinate-\yAdd) {};
\draw[\arrowStyle] (below_grey_1) -- (above_grey_1);
\draw[\arrowStyle] (below_grey_1) -- (central_grey_left);
\draw[\arrowStyle] (blue_below_2_1) -- (below_grey_1);
\draw[\arrowStyle] (blue_below_2_2) -- (central_grey_right);

  \def\xCoordinate{0.0}
  \def\yCoordinate{\yAdd * 2/3}
  \def\x{3.0}
  \def\y{5.0}
  \def\R{\x+0.004}
  \def\yc{\y+0.02}
  \def\e{0.4}
  \def\opacityCones{0.2} 
  
  
  
  
  % blue future cone 1
  \node at (\xCoordinate-\x/2,\yCoordinate-\y*5/6)  {\color{blue} future  cone};
  \begin{scope}[rotate=0]
    \shade[right color=white,left color=blue,opacity=\opacityCones]
      (\xCoordinate-\x,\yCoordinate-\yc) arc (180:360:{\R} and \e) -- (\xCoordinate+\x,\yCoordinate-\yc) -- (\xCoordinate,\yCoordinate) -- cycle;
    \draw[fill=blue,opacity=\opacityCones]
      (\xCoordinate,\yCoordinate-\yc) circle ({\R} and \e);
    \draw[blue, dashed]
      (\xCoordinate-\x,\yCoordinate-\y) -- (\xCoordinate,\yCoordinate) -- (\xCoordinate+\x,\yCoordinate-\y);
    \draw[blue, dashed]
      (\xCoordinate,\yCoordinate-\yc) circle ({\R} and \e);
  \end{scope}
 
 
 
 \def\yCoordinate{-\yAdd * 2/3}
  \def\x{3.0}
  \def\y{6.6}
  \def\R{\x+0.004}
  \def\yc{\y+0.02}
  % red cone 2
   \node at (\xCoordinate+\x*1/2,\yCoordinate+\y*5/6)  {\color{red} past cone};
  \begin{scope}[rotate=0]
    \shade[left color=white, right color=red,opacity=\opacityCones]
    (\xCoordinate-\x,\yCoordinate+\yc) arc (180:360:{\R} and \e) -- (\xCoordinate+\x,\yCoordinate+\yc) -- (\xCoordinate,\yCoordinate) -- cycle;
     \draw[fill=red,opacity=0.3*\opacityCones]
      (\xCoordinate+0,\yCoordinate+\yc) circle ({\R} and \e);
    \draw[red, dashed]
      (\xCoordinate-\x,\yCoordinate+\y) -- (\xCoordinate,\yCoordinate) -- (\xCoordinate+\x,\yCoordinate+\y);
    \draw[red, dashed]
      (\xCoordinate,\yCoordinate+\yc) circle ({\R} and \e);
  \end{scope}
  
\node [single arrow,top  color=red, bottom color=blue,
single arrow head extend=3pt,transform shape, opacity = 2*\opacityCones, minimum height=280pt, text opacity=1, rotate = 270, anchor=west] 
at (\xCoordinate+\x*7/6,\yCoordinate+\y){time
};
 
\end{tikzpicture}
\caption{Future and past cones of a block $x$ in an unstructured DAG}
    \label{fig:conesInTangle}
\end{figure}
